Quality Assessment of Linked Datasets using Probabilistic Approximation

With the increasing application of Linked Open Data, assessing the quality of datasets by computing quality metrics becomes an issue of crucial importance. For large and evolving datasets, an exact, deterministic computation of the quality metrics is too time consuming or expensive. We employ probabilistic techniques such as Reservoir Sampling, Bloom Filters and Clustering Coefficient estimation for implementing a broad set of data quality metrics in an approximate but sufficiently accurate way. Our implementation is integrated in the comprehensive data quality assessment framework Luzzu. We evaluated its performance and accuracy on Linked Open Datasets of broad relevance.

==> sections/extra.tex <==
section 3

\subsection{Dereferenced Backlinks}
%Hogan et al. [Hogan12] describes this metric as the extent to which a local resource URI can be found also as an object in the dataset's triples.
%Therefore, each resource can represent both in-links and out-links.

% * This metric measures the extent to which a resource includes all triples from the dataset that have 
%* the resource's URI as the object. This allows browsers and crawlers to traverse links in either direction, 
% * as specified by Hogan et al. To do so, it computes the ratio between the number of objects that are 
% * "back-links" a.k.a "inlinks" (are part of the resource's URI) and the total number of objects in the resource.
% * 
% * Based on: Hogan Aidan, Umbrich Jürgen. An empirical survey of Linked Data conformance.
%Must detect and dereference all triples where the local URI is mentioned in the object (known as in-links or back-links). The resource may contain millions of such triples, it would take too long to dereference them all. (Use caching or random sampling strategies).
%The problem of detecting the local URI (i.e. the resource's base URI) for big data resources also applies here.
 %detection of all local in-links or back-links: all triples from a dataset that have the resource?s URI as the object [32]
%%
%%Backlinks: The representation should also include all triples from your dataset that have the resource's URI as the object. This is redundant, as these triples can already be retrieved from their subject URIs, but it allows browsers and crawlers to traverse links in either direction.
%%In other words, inlinks can themselves implicitly represent outlinks,36 and inlinks allow for navigating from a given resource to those resources that are related to it.

\subsection{Usage of Unambiguous Annotations}
%remove if implementation is not done
The usage of unambiguous annotations metric measures the degree of which a dataset is clear from ambiguity.
Lei et al.~\cite{Lei2007} describes ambiguous annotation as a quality problem where an instance is mapped to more than one real world object.
A high measure of this metric means that most resources are meaningful and clear.

The easiest way to identify ambiguous resources is to check their \texttt{rdf:type}.
Nonetheless, a resource might have a single type but still refer to the different objects.
In this case a simple approach compares all properties and value of the resource.
%O-notation

%\begin{table}[h]
%\begin{tabular}{|l|l|}
%\hline
%\textit{\textbf{Technique}}                  & \textbf{Metric}                     \\ \hline
%\multirow{2}{*}{\textit{Reservoir Sampling}} & Dereferenceability                  \\ \cline{2-2} 
%                                             & Links to External Data Providers    \\ \hline
%\multirow{2}{*}{\textit{Bloom Filters}}      & Extensional Conciseness             \\ \cline{2-2} 
 %                                            & Unambiguous Annotations             \\ \hline
%\textit{Clustering Coefficient Estimation}   & Clustering Coefficient of a Network \\ \hline
%\end{tabular}
%\end{table}


\begin{algorithm}
\caption{Creating a Reservoir Sampler in Memory}
\label{alg:reservoirSampler}
\begin{algorithmic}[1]
\State set $integer~k$ to the reservoir size
\Function{AddToReservoir}{T item}
\State $n \gets \textit{increment}$
\State $wasAdded \gets \textit{false}$
\State $pos \gets -1$

\If {reservoir is not full up}
\State add item to samplerList
\State $wasAdded \gets \textit{true}$
\Else
\State $pos \gets \textit{random(n)}$
\If {pos $<$ k}
\State remove existing item from samplerList at position $pos$
\State add new item to samplerList at position $pos$
\EndIf
\EndIf
\If {wasAdded}
\State $wasAdded.add(item, pos)$
\EndIf

\Return wasAdded
\EndFunction
\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\caption{Estimated Extensional Conciseness Metric}
\label{alg:estExtCon}
\begin{algorithmic}[1]
\State currentResource $\gets$ ""
\State sortedSetStmt $\gets \emptyset$
\State duplicateInstance $\gets$ 0
\State totalInstance $\gets$ 0

\Function{compute}{Triple t}
\State subject $\gets$ \textit{t.subject()}
\State predicate $\gets$ \textit{t.predicate().toString()}
\State object $\gets$ \textit{t.object().toString()}
\State serialisedStr = predicate." ".object

\If {subject $\neq$ currentResource}
\If {sortedSetStmt $\neq \emptyset$}
\If {RLBSBF.checkDuplicate(sortedSetStmt.toString())}
\State duplicateInstance++
\EndIf
\State sortedSetStmt $\gets \emptyset$
\State currentResource $\gets$ subject
\State totalInstance++
\EndIf
\State sortedSetStmt.add(serialisedStr);
\EndIf
\EndFunction
\end{algorithmic}
\end{algorithm}

\begin{lstlisting}[language=bash,backgroundcolor=\color{white},caption=Convert to n-triples using Jena rdfcat and sort triples in Unix,label=lst:sort]
rdfcat -in RDFXML -out N-TRIPLE file_name > file_name.nt
sort file_name.nt -d -k1,1 -o sorted-file_name.nt
\end{lstlisting}
